Collaborative Uncertainty Benefits Multi-Agent Multi-Modal Trajectory Forecasting

In multi-modal multi-agent trajectory forecasting, two major challenges have not been fully tackled: 1) how to measure the uncertainty brought by the interaction module that causes correlations among the predicted trajectories of multiple agents; 2) how to rank the multiple predictions and select the optimal predicted trajectory. In order to handle these challenges, this work first proposes a novel concept, collaborative uncertainty (CU), which models the uncertainty resulting from interaction modules. Then we build a general CU-aware regression framework with an original permutation-equivariant uncertainty estimator to do both tasks of regression and uncertainty estimation. Further, we apply the proposed framework to current SOTA multi-agent multi-modal forecasting systems as a plugin module, which enables the SOTA systems to 1) estimate the uncertainty in the multi-agent multi-modal trajectory forecasting task; 2) rank the multiple predictions and select the optimal one based on the estimated uncertainty. We conduct extensive experiments on a synthetic dataset and two public large-scale multi-agent trajectory forecasting benchmarks. Experiments show that: 1) on the synthetic dataset, the CU-aware regression framework allows the model to appropriately approximate the ground-truth Laplace distribution; 2) on the multi-agent trajectory forecasting benchmarks, the CU-aware regression framework steadily helps SOTA systems improve their performances. Specially, the proposed framework helps VectorNet improve by 262 cm regarding the Final Displacement Error of the chosen optimal prediction on the nuScenes dataset; 3) for multi-agent multi-modal trajectory forecasting systems, prediction uncertainty is positively correlated with future stochasticity; and 4) the estimated CU values are highly related to the interactive information among agents.

==> 2-Related_Works.tex <==
\section{Related Works}\label{sec:Related_Works}
\textbf{Aleatoric uncertainty estimation in deep learning.}  
Recent efforts are rising as to improve the measurement of aleatoric uncertainty in deep learning models. One seminal work is \cite{NIPS2017_2650d608}. It proposes a unified Bayesian deep learning framework to explicitly represent aleatoric uncertainty using predictive variance for generic regression and classification tasks. Many existing works~\cite{DBLP:conf/cvpr/KendallGC18,ayhan2018test,pmlr-v80-depeweg18a,feng2018towards,wang2019aleatoric,pmlr-v119-kong20b} follow this idea and formulate uncertainty as learned loss attenuation. For example, to make predictive-variance-based aleatoric uncertainty measurements more efficient, \cite{ayhan2018test} adds data augmentation during the test time. But, these works only pay attention to individual uncertainty. 
 
Other recent works attend to the uncertainty measurement for correlated predictive distributions. For example,~\cite{8578672} and \cite{DBLP:conf/nips/MonteiroFCPMKWG20} measure \textit{spatially correlated uncertainty} in a generative model respectively for image reconstruction and pixel-wise classification, and~\cite{hafner2021mastering} captures \textit{joint uncertainty} as discrete variables in the field of reinforcement learning. Despite these three works, our work is the first to conceptualize and measure \textit{collaborative uncertainty} in the multi-agent trajectory forecasting task. To the best of our knowledge, there are only two papers~\cite{DBLP:conf/cvpr/GundavarapuSMSJ19,girgis2021autobots} that are close to our track. \cite{DBLP:conf/cvpr/GundavarapuSMSJ19} and \cite{girgis2021autobots} model the joint uncertainty in the pose estimation task and multi-agent trajectory forecasting task respectively. However, they present several limitations: 1) they did not provide a permutation-equivariant joint uncertainty estimator; 2) they did not provide a theoretical conceptualization or definition of the uncertainty due to correlated predictive distributions; and 3) they did not analyze the causes of such uncertainty. These limitations are essential problems to tackle. Thus, in this work, we not only formulate a general framework with a permutation-equivariant uncertainty estimator, but also theoretically conceptualize \emph{collaborative uncertainty} and analyze its causes.

\textbf{Multi-agent multi-modal trajectory forecasting.} 
%\Note{Yiqi: TODO, focus on describing how existing multi-modal trajectory forecasting works select trajectories. (add some latest related trajectory prediction papers in ref)}
%This task takes the observed trajectories from multiple agents and their surrounding environment (e.g. HD maps) as the inputs, and outputs the predicted trajectory for each agent. A typical deep learning based multi-agent trajectory forecasting system will first encode the inputs as hidden features and decode the features to become the future trajectory of each agent in the scene.
The nature of the trajectory forecasting task is that there are often more than one plausible future trajectory. Recently, multi-modal forecasting has become the dominant research setting in the trajectory forecasting research community~\cite{MemoNet_2022_CVPR,xu2022GroupNet,bae2022npsn,9779572,gu2022stochastic,liang2020learning,zeng2021lanercnn,salzmann2020trajectron++,deo2022multimodal,chai2019multipath,dendorfer2021mg,zhou2022hivt}. This setting requires models to: i) take the observed trajectories from multiple agents and their surrounding environment (e.g., HD maps) as the inputs, and outputs the multiple possible future trajectories predicted for each agent; ii) select the optimal prediction from the predicted trajectories. To tackle the aforementioned requirements, a typical deep-learning-based multi-agent multi-modal trajectory forecasting system usually consists of a regression module that predicts future trajectories and a selection module that ranks the predictions and selects the optimal future trajectory.

In most state-of-the-art (SOTA) forecasting systems, the regression module is designed based on the encoder-decoder architecture. In the encoding process, like many other sequence prediction tasks, the model used to adopt a recurrent architecture to process the inputs~\cite{DBLP:conf/cvpr/AlahiGRRLS16,DBLP:conf/cvpr/HasanSTBGC18,DBLP:conf/cvpr/Liang0NH019}. Later, however, the graph neural networks has become a more common approach as they can significantly assist trajectory forecasting by capturing the interactions among agents~\cite{MemoNet_2022_CVPR,xu2022GroupNet,bae2022npsn,9779572,gu2022stochastic,liang2020learning,https://doi.org/10.48550/arxiv.2102.09117,Ye_2021_CVPR,Yuan_2021_ICCV,hu2020collaborative,https://doi.org/10.48550/arxiv.2202.08408,li2020evolvegraph,DBLP:conf/nips/KosarajuSM0RS19,https://doi.org/10.48550/arxiv.2107.00894}. For the decoding phase, multi-modal forecasting methods usually use multi-layer perceptrons (MLPs) to decode the hidden features~\cite{yagi2018future,robicquet2016learning,lee2017desire,Gao_2020_CVPR}. Many of these methods choose to adopt multiple MLP-based decoders during the decoding phase~\cite{liang2020learning,zeng2021lanercnn,ye2021tpcn}. Each decoder individually predicts one possible trajectory. To ensure the prediction diversity, instead of optimizing all the decoders, those methods tend to only optimize the one that is closest to the ground truth. 

As for the selection module, most SOTA systems are equipped with an MLP-based selector, which assigns the highest confidence score for the prediction that is the closest to the ground truth, to generate a confidence score for each prediction.~\cite{liang2020learning,zeng2021lanercnn,ye2021tpcn,Narayanan_2021_CVPR,Liu_2021_CVPR,Kim_2021_CVPR,song2021learning,gilles2021gohome,gu2021densetnt}.

For safety reasons, it is necessary to report the uncertainty of each predicted trajectory. Works to date about uncertainty measurements ~\cite{DBLP:conf/corl/Jain0LXFSU19,DBLP:conf/cvpr/HongSP19,DBLP:conf/cvpr/LeeCVCTC17,DBLP:conf/eccv/FelsenLG18} have appropriately modeled the interaction among multi-agent trajectories for boosting performances, but they overlook the uncertainty resulting from the correlations in predicted trajectories, and their selection modules do not take the uncertainty of predictions into consideration. We seek to fill these gaps by introducing \emph{collaborative uncertainty} (CU) and designing a CU-based selection module.

%previous use generative model to capture uncertainty(like uncertainty in latent space); not use to select trajectory, like Rules of the Road: Predicting Driving Behavior with a Convolutional Model of Semantic  Interactions also use a score to quantify the possibility of predicted trajectory

==> 4-Experiments_and_Analysis.tex <==
\section{Experiments and Analysis} \label{sec:Experiments}
We first use a self-generated synthetic dataset with a limited number of agents as the toy version of the real-world problem in Subsection~\ref{subsec:syn_data}. We use the simplified dataset to test our method's ability in capturing the distribution information of the input data that obeys the multivariate Laplace distribution, and to evaluate our proposed permutation-equivariant uncertainty estimator. We then conduct extensive experiments on two published benchmarks to prove the value of our proposed method in solving real-world problems in Subsection~\ref{subsec:real_data}. %Moreover, we also manage to disclose the nature of collaborative uncertainty by presenting some additional experimental results in subsection~\ref{subsec:NCU}. Finally, based on our proposed CU-aware regression framework, we study the relationship between prediction diversity and prediction uncertainty in the multi-agent multi-modal trajectory forecasting scenario in subsection~\ref{subsec:D_and_Un}.

\subsection{Toy Problem}
\label{subsec:syn_data}
%\Note{Bh show proofs for 1) why need cu 2) why need permutation equivariant.}
We define a toy problem to validate the capability of the proposed framework in accurately estimating the probability distribution, and to evaluate our permutation-equivariant uncertainty estimator. The toy problem requires models to take the mutually correlated trajectories sampled from the given multivariate Laplace distribution as the input, and output the mean and covariance of this distribution.

As far as we know, in real-world datasets, we only have the ground truth for the predicted trajectory, which is the mean of the distribution, but we do not have access to the ground truth of the uncertainty, which is the covariance matrix of the distribution. Therefore, we generate a synthetic dataset with the ground truth for both the mean and the covariance matrix of the given multivariate Laplace distributions.

\subsubsection{Experimental Setup}
\textbf{Datasets.} We generate a synthetic dataset for the quaternary Laplace distribution. This dataset contains training, validation and test sets, which have 36000, 7000 and 7000 instances respectively. Each instance includes the trajectories of four agents consisting of the two-dimensional point coordinates of the four agents at 50 different timestamps. In each instance, the trajectories of the four agents are sampled from a quaternary joint Laplace distribution. Generation details are provided in Appendix~\ref{ap:TP-GDSD}.

\textbf{Implementation details.} We use the encoder-decoder network architecture for the toy problem. The neural network outputs the predicted mean and covariance matrix of the given quaternary Laplace distribution. Although the ground truth covariance matrix is known in the synthetic dataset, it is not used in training. We train the neural network with the previous uncertainty estimation methods~\cite{NIPS2017_2650d608,tang2021collaborative} and our proposed method respectively. Please find more details in Appendix~\ref{subsec:syn_model}.


\textbf{Metrics.} We adopt four metrics for evaluation: 1) the $\ell_2$ distances between the estimated mean and the ground truth mean, 2) the $\ell_1$ distances between the estimated $\Sigma$ matrix and the ground truth $\Sigma$ matrix, 3) the $\ell_1$ distances between the inverse of the estimated $\Sigma$ matrix and the inverse of the ground truth $\Sigma$ matrix, and 4) the KL divergence between the ground truth distribution and the estimated distribution. We provide the metrics computing details in Appendix~\ref{ap:TP-MCD}.

\begin{table}[t!]
\caption{Comparison with the prior uncertainty estimation framework on the synthetic dataset. \textit{CU} denotes the framework proposed in this paper, \textit{CU-NPE} denotes the framework proposed in~\cite{tang2021collaborative}, and \textit{IU Only} denotes the framework proposed in~\cite{NIPS2017_2650d608}. $\widehat{\mu}$: estimated mean. $\mu_{gt}$: ground truth mean. $\widehat{\Sigma}$: estimated covariance matrix. $\Sigma_{gt}$: ground truth covariance matrix.
$\ell_{2}$ of $\mu$: $||\widehat{\mu} - \mu_{gt}||_{2}$. $\ell_1$ of $\Sigma^{-1}$: $||\widehat{\Sigma}^{-1} - \Sigma^{-1}_{gt}||_{1}$. $\ell_1$ of $\Sigma$: $||\widehat{\Sigma} - \Sigma_{gt}||_{1}$. KL: KL divergence $D_{KL}(p_{g}(\X)||p_{e}(\X))$, where $p_{e}(\X)$ is the estimated distribution and $p_{g}(\X)$ is the ground truth distribution.}\label{tab:simulation_r}
%\vskip -0.5in
\begin{center}
\begin{footnotesize}
\begin{small}{
\begin{tabular}{c|cccc}
\hline
& {$\ell_{2}$ of $\mu$} & {$\ell_1$ of $\Sigma^{-1}$} & {$\ell_1$ of $\Sigma$} & KL \\ \hline
IU Only~\cite{NIPS2017_2650d608} & 0.434  & 0.534    & 0.235    & 4.33  \\ 
CU-NPE\cite{tang2021collaborative}
& 0.376 & 0.502 & 0.209 & 3.15\\
CU
& \textbf{0.359}  & \textbf{0.271}  & \textbf{0.109}  & \textbf{2.11}  \\ 
\hline
\end{tabular}}
\end{small}
\end{footnotesize}
\end{center}
\end{table}

\subsubsection{Results}
\textbf{Quantitative results.} On the test set of our synthetic dataset, we compare the performance of our CU-aware regression framework with the permutation-equivariant uncertainty estimator (CU) and two previous uncertainty estimation frameworks: 1) the framework that only estimates individual uncertainty (IU Only)~\cite{NIPS2017_2650d608}; 2) the framework proposed in~\cite{tang2021collaborative}, which estimates uncertainty via the square-root-free Cholesky decomposition (CU-NPE). Table~\ref{tab:simulation_r} demonstrates that CU allows the model to more accurately estimate the mean and covariance matrix of the given distribution, which leads to a much lower KL divergence between the ground truth distribution and the estimated distribution. 

\textbf{Qualitative results.} Fig.~\ref{fig:permutation} illustrates the outputs of CU and CU-NPE under two different permutations of the same set of inputs, as well as their corresponding ground truths. These visualizations showcase: 1) CU consistently outputs more accurate covariance matrix than CU-NPE; 2) the covariance matrix generated by CU is permutation-equivariant with the input data.


%Besides approximate more accurately, compared with previous, another improvement is that permutation-equivariant. In previous, we estimate via the square-root-free Cholesky decomposition, which includes a lower unit triangular matrix that prevents the generated $\Sigma$ permutation-equivariant with the respect of the input data. Here we provide some empirical proofs.

\begin{figure*}[t!]
\begin{center}
\centerline{\includegraphics[width = 2.\columnwidth]{cus2.pdf}}
\caption{\textbf{Visualization of predicted trajectories.} (a), (b), (c) and (d) show the models' outputs in four different scenarios. The blue line is the past trajectory, the green line is the ground truth future trajectory, and the red lines are predictions generated by the models. The color bar indicates the reliability of each prediction: 1st stands for the most reliable prediction, 2nd for the second most reliable prediction, and so on. In all the four scenarios, predictions generated by the CU-aware LaneGCN is always closer to the ground truth than predictions generated by LaneGCN.}
\label{fig:cus}
\end{center}
\end{figure*}

\subsection{Real-world Problem}
\label{subsec:real_data}
\subsubsection{Experimental Setup}
\textbf{Datasets.} \emph{Argoverse}~\cite{Chang_2019_CVPR} and \emph{nuScenes}~\cite{nuscenes2019} are two widely used multi-agent trajectory forecasting benchmarks. \emph{Argoverse} has over 30000 scenarios collected in Pittsburgh and Miami. Each scenario is a sequence of frames sampled at 10 Hz. The sequences are split as training, validation and test sets, which have 205942, 39472 and 78143 sequences respectively. \emph{nuScenes} collects 1000 scenes in Boston and Singapore. Each scene is annotated at 2 Hz and is 20s-long. The prediction instances are split as training, validation and test sets, which have 32186, 8560 and 9041 instances respectively. For Argoverse, we forecast future trajectories for 3s based on the observed trajectories of 2s. For nuScenes, we forecast future trajectories for 6s based on the observed trajectories of 2s.

\begin{figure*}[t!]
\begin{center}
\centerline{\includegraphics[width = 2.\columnwidth]{v-cu.pdf}}
\caption{\textbf{Visualization of CU on the Argoverse dataset.} (a) In scenario 1, Agent 0, Agent 1 and Agent 2 are respectively located in completely different areas and heading towards different directions; $\sigma_{01}$, $\sigma_{02}$ and $\sigma_{12}$ are close to zero.
(b) In scenario 2, Agent 0, Agent 1 and Agent 2 are driving towards the same direction side by side. This type of scenario may generate complicated interactive information making $\sigma_{01}$, $\sigma_{02}$ and $\sigma_{12}$ show a non-monotonic change over time. (c) In scenario 3, Agent 0 first approaches the road on which Agent 1 is driving, and then moves away from that road, which causes $\sigma_{01}$ to first increase and then decrease. Agent 2 is far away from Agent 0 and Agent 1. Therefore, little new interactive information between Agent 1 and the other two agents would be generated, which makes $\sigma_{02}$ and $\sigma_{12}$ decrease over time.}
\label{fig:cu-v}
\end{center}
\end{figure*}

\textbf{Metrics.} We adopt seven widely used multi-agent trajectory forecasting metrics: $ADE$, $FDE$, $ADE_1$, $FDE_1$, $ADE_k$, $FDE_k$ and $Brier$-$FDE_k$. Firstly, $ADE$ is the Average Displacement Error, i.e., the average of point-wise $\ell_2$ distances between the prediction and the ground truth. Secondly, $FDE$ is the Final Displacement Error, i.e., the $\ell_2$ distance between the final points of the prediction and the ground truth. Thirdly, $ADE_1$/$FDE_1$ is $ADE$/$FDE$ of the selected optimal predicted trajectory Fourthly, $ADE_k$/$FDE_k$ is the minimum $ADE$/$FDE$ of predicted multi-modal trajectories. Finally, $Brier$-$FDE_k$ is the weighted $FDE_k$. (Metrics are in meters. $K=10$ on nuScenes and $K=6$ on Argoverse.)

\begin{table}[tb]
    \centering
    \caption{Comparison with SOTA methods on the Argoverse test set. Collaborative uncertainty estimation boosts performances.}
    %\vspace{-10pt}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{c|ccccccc}
        \hline
        Methods & $ADE_1$ & $FDE_1$ & $ADE_k$ & $FDE_k$ & $Brier$-$FDE_k$\\
        \hline
        GOHOME~\cite{gilles2021gohome} & 1.69 & 3.65 & 0.94 & 1.45 & 1.98\\
        DenseTNT~\cite{gu2021densetnt}  & 1.68 & 3.63 & 0.88 & 1.28 & 1.98\\
        MMTransformer~\cite{liu2021multimodal}  & 1.77 & 4.00 & 0.84 & 1.34 & 2.03\\
        LaneRCNN~\cite{zeng2021lanercnn}  & 1.69 & 3.69 & 0.90 & 1.45 & 2.15\\
        LaneGCN~\cite{liang2020learning}  & 1.71 & 3.78 & 0.87 & 1.36 & 2.06\\
        %LaneGCN (with NPE-CU-aware Regression\cite{tang2021collaborative}) & 1.62 & 3.55 & 0.83 & 1.26 & 1.95\\
        \hline
        CU-aware LaneGCN & \textbf{1.62} & \textbf{3.55} & \textbf{0.83} & \textbf{1.26} & \textbf{1.95}\\
        \hline
    \end{tabular}}
    % \vspace{-10pt}
    \label{tab:with_SOTA}
\end{table}

\textbf{Implementation details.} Here the model is implemented following the CU-aware multi-agent multi-modal trajectory forecasting system illustrated in Section~\ref{sec:Example}. We implement the encoder of LaneGCN~\cite{liang2020learning} and VectorNet~\cite{Gao_2020_CVPR}, which are two cutting-edge multi-agent trajectory forecasting models, as the trajectory encoder in our proposed model. We implement the encoder of LaneGCN based on their official released code.\footnote{LaneGCN official code: https://github.com/uber-research/LaneGCN} At the time of writing, there is no official release of the code for VectorNet yet, and hence we use our self-implemented VectorNet encoder in the experiments. We further use the multi-layer perceptrons to implement $\mu_{\w}(\cdot)$ and $\Phi_{\w}(\cdot)$. Finally, we implement $\Sigma_{\w}(\cdot)$ as the permutation-equivariant uncertainty estimator introduced in Subsection~\ref{subsec:CUUEF}.

\subsubsection{Results}
\textbf{Evaluation results on benchmark.} 
%\Note{Bh show the efficiency of estimating cu via our proposed framework}
For evaluation, we implement our proposed framework based on LaneGCN~\cite{liang2020learning} as it is the SOTA model in multi-agent multi-modal trajectory forecasting. We name the modified LaneGCN that estimates collaborative uncertainty with our proposed CU-aware regression framework as CU-aware LaneGCN. We then compare the performance of CU-aware LaneGCN on the Argoverse trajectory forecasting benchmark with five SOTA methods of this benchmark: GOHOME~\cite{gilles2021gohome}, DenseTNT~\cite{gu2021densetnt}, MMTransformer~\cite{liu2021multimodal}, LaneRCNN~\cite{zeng2021lanercnn}, and LaneGCN~\cite{liang2020learning}. Table~\ref{tab:with_SOTA} demonstrates that the CU-aware LaneGCN especially outperforms all of the competing methods across all chosen metrics. Further, Fig.~\ref{fig:cus} \footnote{In order to keep figures concise, we only visualize the predictions and corresponding ground truths of one agent in each scenario.} visually compares the outputs of LaneGCN and CU-aware LaneGCN, which shows that CU-aware LaneGCN provides more accurate predictions and ranking results than LaneGCN. Therefore, estimating collaborative uncertainty enhances the SOTA prediction model.

\begin{table}[t]
\caption{Comparison with the previous collaborative uncertainty estimation framework in \textbf{\textit{single-modal trajectory forecasting}}. CU denotes the framework proposed in this paper and CU-NPE (None Permutation Equivariant) denotes the framework proposed in~\cite{tang2021collaborative}. $ADE$ and $FDE$ are metrics that evaluate model performance. On both Argoverse and nuScenes, the LaneGCN with CU always outperforms the LaneGCN with CU-NPE.}
\label{tab:single}
%\vspace{-2mm}
%\vskip -0.5in
\begin{center}
\begin{tabular}{c|c|c|cc}
\hline
Method & Dataset & Framework &$ADE$ & $FDE$
\\
\hline
\multirow{2}{*}{} & \multirow{2}{*}{Argoverse}
&CU-NPE & 1.61 & 3.53\\
Single-Modal&&CU& \textbf{1.60} & \textbf{3.52} 
\\
\cline{2-5}
LaneGCN& \multirow{2}{*}{nuScenes}&CU-NPE & 5.27 & 10.55\\
&&CU& \textbf{5.21} & \textbf{10.52}
\\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table*}[t]
\caption{Ablation studies on the uncertainty estimation approach and the interaction module (\textbf{INT.}) in multi-agent multi-modal trajectory forecasting. \textbf{IU} denotes the approach only estimating individual uncertainty. \textbf{IU+CU} denotes our proposed approach that estimates both individual and collaborative uncertainty. On Argoverse and nuScenes, both LaneGCN and VectorNet with individual and collaborative uncertainty estimation surpass the ones with individual uncertainty estimation only. Collaborative uncertainty estimation has a larger impact on the performance of the model with an interaction module.}
%\vspace{-2mm}
\label{tab:ab_in_multi}
%\vskip -0.4in
\begin{center}
\begin{tabular}{c|c|c|cc|c|cc|c|cc|c|cc|c}
\hline
\multirow{2}{*}{Method} &\multirow{2}{*}{Dataset} &\multirow{2}{*}{Int.} & \multicolumn{2}{c|}{$ADE_1$} & \multirow{2}{*}{$\Delta$} & \multicolumn{2}{c|}{$FDE_1$} & \multirow{2}{*}{$\Delta$}& \multicolumn{2}{c|}{$ADE_k$} & \multirow{2}{*}{$\Delta$} & \multicolumn{2}{c|}{$FDE_k$} & \multirow{2}{*}{$\Delta$}
\\
&  & &IU & IU+CU & & IU & IU+CU & & IU & IU+CU &  & IU & IU+CU\\
\hline
\multirow{4}{*}{\scriptsize LaneGCN}&\multirow{2}{*}{\scriptsize Argoverse}&  $\times$ & 1.81 & 1.75 & 3.3\% & 4.18 & 4.02 & 3.8\% & 0.91 & 0.90 & 1.1\% & 1.66 & 1.65 & 0.6\%\\
&&  $\surd$ & 1.33 & \textbf{1.28} & \textbf{3.8\%} & 2.92 & \textbf{2.78} & \textbf{4.8\%} & 0.70 & \textbf{0.69} & \textbf{1.4\%} & 1.03 & \textbf{1.01} & \textbf{1.9\%}
\\
\cline{2-15}
&\multirow{2}{*}{\scriptsize nuScenes}&$\times$ & 7.16 & 6.98 & 2.5\% & 14.74 & 14.34 & 2.7\% & 2.34 & 2.34 & 0.0\% & 3.95 & 3.91 & 1.0\%
\\
&& $\surd$ & 5.53 & \textbf{5.33} & \textbf{3.6\%} & 11.71 & \textbf{10.89} & \textbf{7.0\%} & 1.98 & \textbf{1.82} & \textbf{8.1\%} & 2.90 & \textbf{2.51} & \textbf{13.4\%}
\\
\hline
\hline
\multirow{4}{*}{\scriptsize VectorNet}&\multirow{2}{*}{\scriptsize Argoverse}& $\times$ & 1.80 & 1.80 & 0.0\% & 4.11 & 4.10 & 0.2\% & 1.52 & 1.51 & 0.7\% & 3.35 & 3.32 & 0.8\%
\\
&& $\surd$ & 1.53 & \textbf{1.50} & \textbf{1.9\%} & 3.37 & \textbf{3.31} & \textbf{1.8\%} & 1.32 & \textbf{1.27} & \textbf{4.0\%} & 2.77 & \textbf{2.66} & \textbf{4.0\%}
\\
\cline{2-15}
&\multirow{2}{*}{\scriptsize nuScenes}& $\times$ & 5.02 & 4.41 & 12.2\% & 12.07 & 10.76 & 10.9\% & 1.90 & 1.83 & 3.7\% & 3.84 & 3.67 & 4.4\%
\\
&&$\surd$ & 4.84 & \textbf{3.80} & \textbf{21.5\%} & 11.71 & \textbf{9.09} & \textbf{22.4\%} & 1.77 & \textbf{1.70} & \textbf{4.0\%} & 3.50 & \textbf{3.22} & \textbf{8.0\%}
\\
\hline
\end{tabular}
\end{center}
%\vskip -0.2in
\end{table*}
\label{as_A2A}
\begin{table}[t]
\caption{Ablation studies on the CU-based selection module (CUSelect). For the model without the CU-based selection module, we train an extra neural network to generate the confidence score for it. On both Argoverse and nuScenes, CU-aware models (CU-aware LaneGCN/VectorNet) with the CUSelect always outperform models without it.}
%\vspace{-2mm}
\label{tab:ab_cus}
%\vskip -0.4in
\setlength{\tabcolsep}{1.2mm}{
\begin{center}
\begin{tabular}{c|c|c|cccc}
\hline
Method & Dataset & CUSelect & $ADE_1$& $FDE_1$&$ADE_k$ & $FDE_k$
\\
\hline
&\multirow{2}{*}{Argoverse}&  $\times$ & 1.45 & 3.26 & 0.70 & 1.03\\
CU-aware&&  $\surd$ & \textbf{1.28} & \textbf{2.78} & \textbf{0.69} & \textbf{1.01}
\\
\cline{2-7}
LaneGCN&\multirow{2}{*}{nuScenes}&$\times$ & 6.22 & 12.64 & 1.83 & 2.61
\\
&& $\surd$ &  \textbf{5.33} & \textbf{10.89} & \textbf{1.82} & \textbf{2.51}
\\
\hline
\hline
&\multirow{2}{*}{Argoverse}& $\times$ &1.55 & 3.42 & 1.34 & 2.82
\\
 CU-aware&& $\surd$ & \textbf{1.50} & \textbf{3.31} & \textbf{1.26} & \textbf{2.67}
\\
\cline{2-7}
VectorNet&\multirow{2}{*}{ nuScenes}& $\times$ & 5.89 & 14.14 & 1.88 & 3.82
\\
&&$\surd$ & \textbf{3.80} & \textbf{9.09} & \textbf{1.70} & \textbf{3.22}
\\
\hline
\end{tabular}
\end{center}}
%\vskip -0.2in
\end{table}

\textbf{Evaluation results for single-modal forecasting.} To compare our proposed CU-aware regression framework (CU) and the previous collaborative uncertainty estimation framework (CU-NPE) proposed in~\cite{tang2021collaborative} under the multi-agent trajectory forecasting setting. We generalize LaneGCN to the single-modal scenario by letting the forecasting module only predict one possible future trajectory for each agent and removing the selection module. Table~\ref{tab:single} shows that, on the test set of both Argoverse and nuScenes, the single-modal LaneGCN with CU always outperforms it with CU-NPE. We speculate that this improvement may come from the permutation-equivariant uncertainty estimator, which makes the uncertainty estimation more accurate.


\textbf{Visualization of collaborative uncertainty.} To visually understand which factor influences the value of CU in multi-agent multi-modal trajectory forecasting, Fig.~\ref{fig:cu-v} illustrates the visualization results generated by our model. We visualize three scenarios. Each scenario includes three agents' trajectories (i.e., orange, blue and green dash lines) and their corresponding CU values changing over the last 30 frames (i.e., the heatmap, where $\sigma_{ij}$ denotes the CU of agent $i$ and agent $j$). The visualization results show that the value of CU in multi-agent multi-modal trajectory forecasting is highly related to the interactive information among agents.\footnote{Note that to keep the visualization results concise, for each scenario, we only visualize the optimal trajectory and its corresponding CU.}

%\textbf{Visualization of predicted trajectories.}

%\textbf{Visualization of the CU-based selection.} Fig.~\ref{} shows how the proposed CU-based selection module works in the real world application. 

\subsubsection{Ablation Study}
\label{subsec:ab}
We study: 1) how different approaches of uncertainty estimation would impact the prediction model; 2) how the proposed CU-based selection module would affect the CU-aware multi-modal trajectory forecasting system; 3) how the proposed auxiliary uncertainty training loss (AUTL) would influence the performance of the CU-aware regression framework in multi-modal trajectory forecasting. In this part, we adopt LaneGCN/VectorNet as our trajectory encoder for proving that our proposed method can be used as a plug-in module to improve the performance of existing models for multi-agent multi-modal trajectory forecasting. Here, experiments are conducted on the validation sets of the Argoverse and nuScenes benchmarks.

\textbf{Effect of different uncertainty estimation approaches.} In the multi-agent multi-modal trajectory forecasting task, on the basis of LaneGCN/VectorNet, we consider two approaches of uncertainty estimation: 1) estimating individual uncertainty only (IU); 2) estimating both collaborative and individual uncertainty (IU + CU). Table~\ref{tab:ab_in_multi} demonstrates that estimating both individual and collaborative uncertainty (IU + CU) is consistently better than estimating individual uncertainty only (IU). These results reflect that our collaborative uncertainty estimation (i.e., the CU-aware regression framework) can function as a plugin module to improve the prediction performance of existing models. %\textit{Further, Appendix~\ref{sec:CWCUCD} demonstrates that the CU-aware framework can outperform our previous collaborative uncertainty estimation method~\cite{tang2021collaborative} in the single-modal trajectory forecasting.}

\textbf{Effect of the CU-based selection module.} Here, we empirically study how the proposed CU-based selection module influences the CU-aware multi-agent multi-modal trajectory forecasting system. For the model without the CU-based selection module, we train an extra neural network to generate the confidence score for each predicted trajectory. Table~\ref{tab:ab_cus} shows that, the forecasting model with the CU-based selection module always provides more accurate results than the model without it, which indicates that our CU-based selection module improves the performance of the CU-aware forecasting model.

\begin{table}[t!]
\caption{Ablation studies on auxiliary uncertainty training loss (AULT) in CU-aware multi-modal trajectory forecasting models (CU-aware LaneGCN/VectorNet). $\Delta$ represents the improvement that AUTL brings to the forecasting model. On both Argoverse and nuScenes, AUTL benefits the prediction model, and it impacts $ADE_1/FDE_1$ significantly, more so than it impacts $ADE_K/FDE_K$.}
%\vspace{-2mm}
\label{tab:AUTL}
\begin{center}
\begin{tabular}{c|c|c|cc|c}
\hline
\multirow{2}{*}{Method} &\multirow{2}{*}{Dataset} &\multirow{2}{*}{Metrics} & \multicolumn{2}{c|}{AULT} & \multirow{2}{*}{$\Delta$}
\\
&  & &$\times$ & $\surd$ & \\
\hline
\multirow{3}{*}{}&\multirow{4}{*}{ Argoverse}&  $ADE_K$ & 0.70 & \textbf{0.69} & 2.6\%
\\
 &&  $ADE_1$ & 1.42 & \textbf{1.28} & \textbf{9.6\%}
\\
\cline{3-6}
&&  $FDE_K$ & 1.06 & \textbf{1.01} & 5.1\%
\\
CU-aware&&  $FDE_1$ & 3.14 & \textbf{2.78} & \textbf{11.4\%}
\\
\cline{2-6}
LaneGCN&\multirow{4}{*}{nuScenes}&  $ADE_K$ & 1.84
 & \textbf{1.82}
 & 1.4\%
\\
\multirow{3}{*}{}&&  $ADE_1$ & 11.40
 & \textbf{5.33}
 & \textbf{53.3\%}
\\
\cline{3-6}
&&  $FDE_K$ & 2.57
 & \textbf{2.51}
 & 2.2\%
\\
&&  $FDE_1$ & 23.39
 & \textbf{10.89}
 & \textbf{53.4\%}
\\
\hline
\hline
\multirow{3}{*}{}&\multirow{4}{*}{ Argoverse}&  $ADE_K$ & 1.30
 & \textbf{1.27}
 & 3.0\%
\\
&&  $ADE_1$ & 2.40
 & \textbf{1.50}
& \textbf{37.4\%}
\\
\cline{3-6}
&&  $FDE_K$ & 2.75
 & \textbf{2.66}
 & 3.3\%
\\
CU-aware&&  $FDE_1$ & 5.50
 & \textbf{3.31}
 & \textbf{39.8\%}
\\
\cline{2-6}
VectorNet&\multirow{4}{*}{nuScenes}&  $ADE_K$ & 1.79
 & \textbf{1.70}
 & 5.3\%
\\
\multirow{3}{*}{}&&  $ADE_1$ & 4.86
 & \textbf{3.80}
 & \textbf{21.8\%}
\\
\cline{3-6}
&&  $FDE_K$ & 3.55
 & \textbf{3.22}
 & 9.3\%
\\
&&  $FDE_1$ & 11.79
 & \textbf{9.09}
 & \textbf{22.9\%}
\\
\hline
\end{tabular}
\end{center}
\end{table}
\label{as_A2A}

\textbf{Effect of the auxiliary uncertainty training loss (AUTL).} The ablation study results on the proposed AUTL are shown in Table~\ref{tab:AUTL}. Results show that CU-aware models (CU-aware LaneGCN/VectorNet) trained with AUTL always outperform CU-aware models trained without it on all chosen metrics, and that AULT makes a larger improvement in $ADE_1/FDE_1$ than in $ADE_K/FDE_K$. These results show a proof that the proposed AUTL benefits CU-aware multi-agent multi-modal trajectory forecasting models, especially in terms of choosing the optimal predicted trajectory. 

\begin{figure*}[t]
\begin{center}
\centerline{
\includegraphics[width=1.8\columnwidth]{sto-un2.pdf}}
%\vskip -0.1in
\caption{\textbf{Relationship between future stochasticity and the prediction uncertainty (i.e., the stochasticity-uncertainty relationship)} for (a) LaneGCN: LaneGCN on the Argoverse dataset and the nuScenes dataset, (b) VectorNet: VectorNet on the Argoverse dataset and the nuScenes dataset. These results show a positively correlated stochasticity-uncertainty relationship.}
%\vskip -0.3in
\label{fig:diver-un}
\end{center}
\end{figure*}
\begin{figure*}[t!]
\begin{center}
\centerline{\includegraphics[width = 1.8\columnwidth]{compa_inc2.pdf}}
\caption{\textbf{CU estimation gains more when a prediction model includes interaction modeling.} Blue and red bars reflect the gains from CU estimation for a prediction model with/without an interaction module respectively. $\Delta FDE_1$/$\Delta FDE_k$ are the improvement rate of $FDE_1$/$FDE_k$ between versions with/without CU estimation respectively. Data of this figure comes from experiments on the nuScenes dataset shown in Table~\ref{tab:ab_in_multi}.}
\label{fig:comp_in}
\end{center}
\end{figure*}

\section{Discussion: What Causes the Uncertainty in Multi-Agent Multi-Modal Trajectory Forecasting}
\label{sec:discussion}
In Section~\ref{sec:Experiments}, our experimental results show that the CU-aware regression framework can be used to aid models in approximating the distribution information of given data and in improving prediction performance. In this section, we leverage the proposed CU-aware regression framework to study the cause of the uncertainty in multi-agent multi-modal trajectory forecasting, particularly the cause of our proposed collaborative uncertainty.

\subsection{Cause of Uncertainty}
\label{subsec:D_and_Un}
As mentioned in Section~\ref{sec:Related_Works} and Section~\ref{sec:Methodology}, potential future trajectories of multiple agents are inherently stochastic. We argue that future stochasticity contributes to the uncertainty in multi-agent multi-modal trajectory forecasting. 

To support this argument, we empirically study the relationship between future stochasticity and the prediction uncertainty (i.e., the stochasticity-uncertainty relationship) of multi-agent multi-modal trajectory forecasting models. In our experiments, the prediction uncertainty is quantified by our proposed Laplace CU-aware regression framework. For the scale of future stochasticity, according to \cite{DBLP:journals/corr/abs-1911-12736} and \cite{yuan2020dlow}, the prediction diversity of a forecasting model is positively correlated with the stochasticity of given agents' potential future trajectories. Therefore, we use the prediction diversity of multi-agent multi-modal trajectory forecasting systems to estimate the future stochasticity scale, which can be quantified by (\ref{eq:DS}).

\begin{equation}
\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}
    {\rm Stochasticity} =  m( \frac{\sum\limits_{i=1}^{K}(\widehat{\mu}_i - \overline{\widehat{\mu}})^{2}}{K-1}),
    \label{eq:DS}
\end{equation}
where $\widehat{\mu}=[\widehat{\mu}_{1}, \widehat{\mu}_{2}, ..., \widehat{\mu}_{K}]$ is a multi-modal prediction result, $K$ is the number of the prediction modal, $\widehat{\mu}_{k} \in \R^{2T_{+}}$, $\overline{\widehat{\mu}} \in \R^{2T_{+}}$ is the mean of elements in $\widehat{\mu}$, and $m(\cdot)$ symbolizes the computation of element-wise average of a vector.

We visually analyze the stochasticity-uncertainty relationship for LaneGCN as well as VectorNet on the Argoverse and nuScenes datasets. See visualization results in Fig.~\ref{fig:diver-un}. These results show a positive correlation between future stochasticity and prediction uncertainty in multi-agent multi-modal trajectory forecasting models. Therefore, the stochasticity of given agents' potential future trajectories contributes to the existence of uncertainty in multi-agent multi-modal trajectory forecasting.

%To the best of our knowledge, our work is the first to quantitatively study the diversity-uncertainty relationship in trajectory forecasting. We hope that the positively correlated diversity-uncertainty relationship, as disclosed by this work, can inspire other researchers in this area. For example, one theoretical implication of this correlation is that future works can try to make prediction diversity adjustable for each scene according to its model uncertainty.

\subsection{Cause of Collaborative Uncertainty}
\label{subsec:NCU}
In this subsection, we focus on the cause of our proposed collaborative uncertainty. As mentioned in Section~\ref{sec:problem_formulation}, we can divide multi-agent multi-modal trajectory forecasting models into two types: the individual model and the collaborative model. The individual model predicts the future trajectory and the corresponding uncertainty for each agent independently, while the collaborative model leverages an interaction module to explicitly capture the interactions among multiple agents, which makes all the predicted trajectories correlated. The correlations among predicted trajectories can bring extra uncertainty to the model; in other words, we consider that the interaction module in a forecasting model leads to collaborative uncertainty.

To validate this, we empirically compare the impact of collaborative uncertainty estimation on an individual model versus a collaborative model. In our experiments, we use two cutting-edge multi-agent trajectory forecasting models, LaneGCN~\cite{liang2020learning} and VectorNet~\cite{Gao_2020_CVPR}. Furthermore, the improvement rate of $ADE_1$, $FDE_1$, $ADE_k$, and $FDE_k$ between models with/without an interaction module are represented by $\Delta ADE_1$, $\Delta FDE_1$, $\Delta ADE_k$, and $\Delta FDE_k$ respectively. As Fig.~\ref{fig:comp_in} illustrates, when we remove the interaction module from LaneGCN/VectorNet, collaborative uncertainty estimation brings much less gain to LaneGCN/VectorNet (see Table~\ref{tab:ab_in_multi} for more results of this experiment). As a result, the interaction module causes the collaborative uncertainty in multi-agent multi-modal trajectory forecasting.
